A Complex KBQA System using Multiple Reasoning Paths

Multi-hop knowledge based question answering (KBQA) is a complex task for natural language understanding. Many KBQA approaches have been proposed in recent years, and most of them are trained based on labeled reasoning path. This hinders the system's performance as many correct reasoning paths are not labeled as ground truth, and thus they cannot be learned. In this paper, we introduce an end-to-end KBQA system which can leverage multiple reasoning paths' information and only requires labeled answer as supervision. We conduct experiments on several benchmark datasets containing both single-hop simple questions as well as muti-hop complex questions, including WebQuestionSP (WQSP), ComplexWebQuestion-1.1 (CWQ), and PathQuestion-Large (PQL), and demonstrate strong performance.

==> Introduction.tex <==
\begin{figure}[t]
 \centering
 \includegraphics[width=1\linewidth]{figs/fig1.png}
 \caption{One QA example with Multiple Relation Paths from \textsc{ComplexWebQuestion}-1.1. The blue color highlighted is the extracted topic entity. Each square represents an entity, and the arrows represent the relations. Relation path $R_1$ to $R_4$ are the good ones containing meaningful relation paths to the final answer. $R_5$ and $R_6$ are the worse paths that generate a larger final answer set containing some wrong entities. $R_7$ is the worst one as its relation path is totally not interpretable and the answer set is huge.}
 \label{QAPaths}
\end{figure}

\section{Introduction}

Knowledge-based question answering (KBQA) is the task of finding answers to questions by processing a structured knowledge base $\mathcal{KB}$. %where the beliefs are stored as triples containing two entities and the relation linking them. 
A $\mathcal{KB}$ consists of a set of entities $\mathcal{E}$, a set of relations $\mathcal{R}$, and a set of literals $\mathcal{S}$ \cheng{and as set of facts?}. A knowledge base fact is defined as $(h,r,t)$, where $h\in \mathcal{E}$ is the head entity, $t \in \mathcal{E} \bigcup \mathcal{S}$ is the tail entity/literal \cheng{when do we use literals?}, and $r\in \mathcal{R}$ is the directed relation between $h$ and $t$. To answer a simple single-relation question (\emph{i.e.} a 1-hop question) such as: ``Who is the president of the United States?'', %a KBQA system first identifies the topic/focus entity (\emph{i.e.} United States) and the relation (\emph{i.e.} ``president '') asked in the question, then searches for the entity by matching the entity-relation tuple $\textless$United States, president, $?\textgreater$ over KB. \kalpa{use of a topic entity is approach specific. Many KBQA systems exist that do not use topic entity. E.g., template based QA}
a typical KBQA system first identifies the entity (\emph{i.e.} United States) and the relation (\emph{i.e.} ``president'') asked in the question, and then searches for the answer entity by matching the entity-relation tuple $\textless$United States, president, $?\textgreater$ over $\mathcal{KB}$.


While the single-hop question can be answered by searching a predicate relation in $\mathcal{KB}$, it is much harder to answer more complex multi-hop questions containing multiple entities and relations with constraints. For instance, for complex compositional questions, it is not easy to extract all the correct relations together withhead and tail entities in the right order. For complex conjunction questions \cheng{need to explain what conjunction question means}, it is often difficult to extract all the reasoning paths involved, and combine their results in the end. 

Most prior work on multi-hop KBQA focuses on learning the single given ground truth relation path for each question, and outputting  the most possible reasoning path during prediction \cheng{we need to unify "reasoning path" and "relation path"}. In reality, however, it is often the case that there exist many alternative relation paths that all lead to the correct answer, and these are not provided as ground truth by the human annotators. %It is hard to pre-define the maximum number of hops in a complex question because different questions may need different number of hops to reach their answers.
%\kechen{list a few problems (1) it hard to control number of hops. (2) how to decompose a complex question into sub-question. (3) ...} 
%\kechen{add something to explain why the above two points lead to decomposing into two sub-tasks?}
 %with random walks \cite{DBLP:conf/emnlp/GardnerTKM13} or is formulated as a Markov decision process (MDP) based reinforcement learning problem~\cite{DBLP:conf/emnlp/XiongHW17}.
%\kechen{Most of the existing KBQA systems cannot handle these two issues simultaneously. People have to pre-define different rules to solve different type of complex querys. For example, list a few work using different pre-defined strategy to solve complex QA.}%1. use different model to train, 2. neural program
%traditional approaches consider all the paths and search for the best path among them, where their searching algorithms either leverage path-ranking algorithms with random walks \cite{DBLP:conf/emnlp/GardnerTKM13} or is formulated as a Markov decision process (MDP) based reinforcement learning problem~\cite{DBLP:conf/emnlp/XiongHW17}. Since the complexity of the searching process can grow exponentially when the number of hops increase, some recent researches add decision markers or a terminal relation to decide whether a searching path should terminate or continue, in order to reduce the searching space and complexity \cite{DBLP:conf/naacl/ChenCCNK19}.
%It is commonly observed that, by using the above mentioned algorithms, the extracted relation path may not always be the best one or even can be a wrong one. The main reason is because during training, for one question, their models are trying to learn and fit to only one possible relation path, which is given as its ground truth. \kechen{while during prediction only predict one path}In reality, however, it is always possible that there exists many other relation paths leading to the answer, which are not given as ground truth. 
For example, Figure \ref{QAPaths} shows 7 relation paths $R_n={e^n_0\rightarrow r^n_1 \rightarrow e^n_1 \rightarrow \cdots \rightarrow e^n_{ans}}\ (n=\lbrace 1, \dots, 7 \rbrace)$ leading to the correct answer entity ``West Lafayette'' for the question \textit{``What city is home to the University that is known for Purdue Boilermakers men's basketball?''} %\footnote{An exchangeable way to define relation path is omitting entities in the definition, because entity is determined by given the topic entity, relations, and the knowledge base. For simplicity, we simplify this relation path definition as a list of sequential relations $(r_{1}^n, r_{2}^n, \cdots, r_{T}^n)$ in the following part of this paper.}
, but only the relation path R1 is labeled as the ground truth relation path in the dataset. \cheng{These statements are too general and speculative. Better to explain with concrete failure cases.} \fix{It is unlikely for the model to infer all possible relation paths that can direct the model to the answer set containing the final answer, only based on one given training path. It is not even possible for the model to differentiate the good paths from the bad ones, which are some unreasonable paths also leading to the answer sets %containing our target answer
or some reasonable paths leading to a large predicted set which contains both correct answer and noisy results.} \cheng{We need to first explain what we mean by good paths, which are good paths, and then claim that existing methods cannot disinguish good ones from bad ones} As the example given in Figure \ref{QAPaths}, relation paths $R_1$ to $R_4$ are the good ones containing meaningful relation paths to the final answer, by executing different number of hops. \cheng{We cannot simply define good paths as "meaningful" paths. This is not a useful definition. Define a good path as a path that leads to a small answer set?} Comparatively, relation paths $R_5$ and $R_6$ lead to a larger final answer set containing not only the correct answer entity but also many other wrong entities. These paths can be treated as inferior to the top 4 paths, since they give some extra invalid answers besides the correct one. \cheng{It is not clear where the discussion on good path vs bad path comes from. Why do I need to care about good path vs bad path? Who set this standard for good path? Is that us, or is that implied by the f1 evaluation metric? Is that for better interpretability?} In the example, path $R_7$ is even worse as its relation path is totally not interpretable plus the final answer set is exaggeratedly large which mainly contains invalid answers, hence should not be considered as a positive relation path training sample for this question. \cheng{Here we need a summary of why existing methods are bad}

%Although someone may claim that we can use multiple relation paths as ground truths for one question to improve the coverage and performance, it is still not feasible to label all valid relation paths considering the complexity of ground truth label preparation. 
%\kechen{combine this paragraph with the next paragraph? now we have two separate paragraphs to first introduce the issue and then use an example to explain it. should we combine them together?}

In this paper, we propose an end-to-end multi-hop KBQA system, which can leverage the training information from multiple relation paths, and learn the good relation paths over the inferior or the bad ones, based on only one given relation path annotation per instance (as in most KBQA datasets) or even no relation path annotation. We model the relation path as a latent variable, and propose supporting training and prediction methods. Experimental results show that the system can output diverse relation paths, and reward the ``better'' paths over the inferior ones by assigning ``better'' paths higher probabilities. Our method can be applied to most KBQA systems to predict entity and relation, and can be used with any model architecture. We achieve strong performance on three popular KBQA datasets for single-hop and multi-hop questions. \kechen{Especially, we show that our model perform extremely well on difficult dataset vs. simple dataset, multi-hop question vs. single question, and multiple path question vs. single path question.} %taking the size of their answer set into consideration, \emph{i.e.} the larger is the final answer set, the worse is a relation path, as it contains more irrelevant answer information. \kechen{modify the last sentence} %We also use a sampling approach to filter the wrong paths like $R_8$ in our example. 
% Specifically, we make the following contributions:\\
% 1. We introduce a novel multi-hop KBQA structure, which can predict the relation sequence of any length without pre-defining the number of maximum hops and generate final answers at the last hop.\\
% 2. We design a novel loss function using latent variables, such that the system can be trained without being given any ground truth relation path, or by leveraging more valid training paths information even if one ground truth path is given. We also give detailed analysis to demonstrate the benefits of using the new loss function.\\
% 3. We achieve state-of-the-art performance on three popular KBQA dataset containing single-hop and multi-hop questions.
%Specifically, we make the following contributions:
%\begin{enumerate}
%    \item We introduce a novel multi-hop KBQA system, which can leverage the information from multiple relation paths. %predict the relation sequence of any length without pre-defining the number of maximum hops and generate final answers at the last hop.
%    \item We design a novel loss function and the corresponding training and prediction methods. Detailed analysis is given to demonstrate the benefits of using this new loss function.
%    \item We achieve state-of-the-art performance on three popular KBQA datasets for single-hop and multi-hop questions.
%\end{enumerate}


==> backup.tex <==
\begin{table*}[h]\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
                            & PQL2 & PQL3 & PQL+ & WQSP & CWQ \\
\hline
KV-MemNN \cite{DBLP:conf/emnlp/MillerFDKBW16}    & 72.2 & 67.4 & -    & 46.7 / - & 21.1\footnote{The original paper only reports scores on development set.} / -      \\
IRN \cite{DBLP:conf/coling/ZhouHZ18}                         & 72.5 & 71.0   & 52.9 & -    & -         \\
HR-BiLSTM \cite{DBLP:conf/acl/YuYHSXZ17}                  & 97.5 & 87.9 & 92.9 & 62.9 / 62.3 & 33.3 / 31.2         \\
ABWIM \cite{DBLP:journals/corr/abs-1801-09893}                      & 94.3 & 89.3 & 92.6 & -    & -         \\
UHop\footnote{We use the best reported setup from the original paper, aka. ABWIM with UHop.} \cite{DBLP:conf/naacl/ChenCCNK19}                       & 97.5 & 89.3 & 92.3 & -    & -         \\
GRAFT-Net \cite{DBLP:conf/emnlp/SunDZMSC18}                  & -    & -    & -    & 67.8 / 62.5 & 30.1 / 26.0      \\
KBQA with Topic Units \cite{DBLP:conf/ijcai/LanW019}                  & -    & -    & -    & 68.2 / 67.9 & 39.3 / 36.5      \\
\hline
Our Method-obj1             & 98.3 & 97.1 & 97.5 &    62.8 / 62.3  &           \\
Our Method-obj2             &   -   &   -   &   -   &  65.4 / 65.1     &           \\
Our Method-obj3             &     - &  -    &   -   &   67.9 / 67.0    &           \\
Our Method-obj3+new\_decode & -     &   -   &    -   &     &          \\
\hline
\end{tabular}
\caption{\fontsize{10}{12}\selectfont We report Accuracy on PQL and hits@1 and F1 on WQSP and CWQ. All scores except our method are copied from the previous published papers. obj1/2: $P(ans, path|x)= P(ans|path,x)*P(path|x)$ with single/multiple reasoning paths for one sample. obj3: $P(ans) = sum_path(P(ans|path,x)*P(path|x))$, new\_decode: use beam search and multi paths in decoding.}\label{tab:main}
\end{table*}


\begin{figure}[h]
\centering
\includegraphics[width=0.85\columnwidth]{figs/fig2.png}
\vspace{-2ex}
\caption{\fontsize{10}{12}\selectfont Average F1 over different thresholds on \textsc{WebQuestionSp} dataset.}
\label{fig:k2}
\end{figure}


\begin{table}[h]\centering
\resizebox{1.01\columnwidth}{!}{
\begin{tabular}{|l|c|c|}
\hline
                           & WQSP & CWQ \\
\hline
%KV-MemNN \cite{DBLP:conf/emnlp/MillerFDKBW16}    & 46.7 / - & 21.1\tablefootnote{The original paper only reports scores on development set.} / -      \\
HR-BiLSTM \cite{DBLP:conf/acl/YuYHSXZ17}                  & 62.9 / 62.3 & 33.3 / 31.2         \\
GRAFT-Net \cite{DBLP:conf/emnlp/SunDZMSC18}                & 67.8 / 62.5 & 30.1 / 26.0      \\
KBQA-GST \cite{DBLP:conf/ijcai/LanW019}          & 68.2 / 67.9 & 39.3 / \textbf{36.5}      \\
\hline
Our Method-joint\_prob             &    62.8 / 62.3  &   36.7 / 31.4        \\
Our Method-joint\_prob\_multiple\_paths             &  65.4 / 65.1     &    - / -       \\
Our Method-marginal\_prob\_with\_true\_label             &   \textbf{68.9} / \textbf{68.5}    &      \textbf{39.4} / 34.8     \\
Our Method-marginal\_prob\_without\_true\_label             &   68.8 / 68.3    &       33.0 / 27.6    \\
%Our Method-obj3+new\_decode  &     &          \\
\hline
\end{tabular}
}
\caption{\fontsize{10}{12}\selectfont We report hits@1 / F1 on WQSP and CWQ.}\label{tab:wqsp_cwq}
\end{table}


A general neural network solution to KBQA is to encode the candidates of relation path or answer into embeddings, and choose or rank these embeddings based on different ranking functions. Existing approaches can be categorized into three types. One is to match the question to a candidate directly via calculating the similarity between them \cite{DBLP:journals/corr/abs-1801-09893,DBLP:conf/adbis/YuHYZW18}. This method is not very suitable for multi-hop questions with long paths, because the number of candidate entity-relation combinations grows exponentially as the number of hops increases. The second type of algorithms is to encode the reasoning information hop by hop, and predict the final answer at the last hop \cite{DBLP:conf/emnlp/MillerFDKBW16,DBLP:conf/coling/ZhouHZ18}, which is a group of methods that are more capable of handling multi-hop questions. Most of these algorithms, however, are restricted to a fixed maximum number of hops, and this number is normally chosen as a relative small number. Recently, a new unrestricted-hop framework is proposed to dynamically choose the number of hops to be executed, by introducing a ``stop'' action to decide when is the last hop \cite{DBLP:conf/naacl/ChenCCNK19}. The third type is specifically designed for multi-hop KBQA, which decompose the input question into several single-hop question, and use the exiting method to solve each simple question. The decomposition methods are based on semantic parsing \cite{DBLP:conf/www/AbujabalYRW17,DBLP:conf/emnlp/LuoLLZ18}, pointer network \cite{DBLP:conf/acl/MinZZH19}, or predefined templates \cite{DBLP:journals/pvldb/ZhengYZC18,DBLP:journals/corr/abs-1807-09623}.  %This number is normally chosen as a relative small number like 1 (single hop), 2 or 3. One main reason is because that, despite theoretically it is possible to search all the possible relations greedily and find the paths starting from the focus entity in the question to the answer entity, the number of all possible entity-relation combinations grows exponentially. It is unrealistic to store or even enlist all these paths when the number of hops is too large. Moreover, it is also unlikely for the system to know the number of hops in advance in real applications. 
 To further improve a multi-hop KBQA system's performance, some recent work also replaces the standard entity linking module by leveraging an augmented topic entity candidate pool \cite{DBLP:conf/ijcai/LanW019}, such that it can cover more entity possibilities. This work is similar to our idea that making use of multiple input information to train the model, but their focus is on entities while ours is on relation paths.
%\kechen{add relation prediction references and multiple relation path, recent ijcai paper?}



\kechen{should we move this to RW? Most of the existing multi-hop KBQA systems \cite{DBLP:conf/acl/YuYHSXZ17,DBLP:journals/corr/abs-1801-09893,DBLP:conf/coling/ZhouHZ18,DBLP:conf/naacl/ChenCCNK19} approach this task by decomposing it into two sub-tasks:
%Currently, there are mainly two main categories of methods to tackle the complex KBQA problems, the first category is based on semantic parsing, and the other category mainly relies on the embeddings (XXX) for information retrieval (IR). %Their differences will be discussed further in the relation work section, and i
%In this paper, we focus on the second category, \emph{i.e.} the embedding based approach, which can either predict the answer directly (XXX) or search (a) relation path(s) leading to the final answer entity (XXX). Conventionally, the relation path searching algorithm consists two main subtasks
topic/focus--entity linking and relation extraction. The topic--entity linking gives the system an entry point to start searching, and the relation extraction is used to search relation paths leading to the final answer. %Unlike the simple single relation questions, for complex questions, the path to the final answer may contains multiple hops, where one hop is defined as a searching step between one entity to another via a single relation. 
For entity linking, there exists many off-the-shell tools  \cite{DBLP:journals/corr/YangC16a} that can give decent performance, and most of the current KBQA models rely on them. For relation extraction, traditional approaches consider all the paths as candidates and search for the best one among them using ranking algorithms.}


We also implement a baseline version of our method with only the question encoding and relation prediction modules. By removing entity lookup and answer prediction modules, our model works similarly as a vanilla RNN model with attention. The baseline model generates a sequence of relations and uses them to fetch the final answer from the knowledge base by following them sequentially. By comparing the last two rows in Table \ref{tab:qpl}, we can see that, by adding the entity lookup module, there is a significant performance boost. It equips our model with the ability not only to search but also to interact with the knowledge base. It can be further observed for Table \ref{tab:qpl} that our model performs much better than the conventional KV-MemNN, which has an entity lookup module, but does not contain a relation prediction module. We believe that this is because the intermediate key-value operations benefit from the direct relation supervision. Therefore, our model can be treated as a good combination of RNN-attention model and KV-MemNN. 


\subsubsection{WebQuestionSP \& ComplexWebQuestion-1.1}
\kechen{only report marginal prob in table 2 and move others to table 3}

\textsc{WebQuestionSP} is a dataset that has been widely used for relation extraction and end-to-end KBQA task. It contains 1 or 2 hops questions with ground truth relation path labels. Table \ref{tab:wqsp_cwq} shows that our model with marginal training objective performs much better than all other methods. KBQA-GST \cite{DBLP:conf/ijcai/LanW019} relies on additional annotations, such as textual description of the knowledge base, and using existing models to generate features. The experiments from their papers show that these generated extra features play a very important role in the system, and their F1 score drops from 67.9 to 61.5 by removing the semantic feature. Similarly, HR-BiLSTM requires relation path annotations to train their model, which are not accessible in many KBQA application scenarios. In contrast, our model supports a training method that takes only raw QA pairs as its input and does not rely on any additional labels or linguistic features. By comparing performance of using different objectives as shown in the second block of the table, we can see that there is a significant improvement by considering multiple relation paths in training. The performance gap between joint objective and marginal objective demonstrates that our proposed marginal objective is a much better way to train a model with multiple relation paths. We do not observe a very different results by using or not using labeled relation paths, which is a good signal. 
Previous stateof-the-art method NSM is only tested on a single dataset. It is unclear whether they could perform consistently well on different datasets. Our full model is shown to consistently work well on three datasets.

\begin{table}[h]\centering
\resizebox{1.01\columnwidth}{!}{
\begin{tabular}{|l|c|c|}
\hline
                           & WQSP & CWQ \\
\hline
KV-MemNN* \cite{DBLP:conf/emnlp/MillerFDKBW16}    &  38.6 &  -      \\
STAGG\_answer* \cite{DBLP:conf/acl/YihRMCS16}  &  66.8 &  -      \\
NSM* \cite{DBLP:conf/acl/LiangBLFL17}  &  69.0 &  -      \\
GRAFT-Net* \cite{DBLP:conf/emnlp/SunDZMSC18}                &  62.8 &  26.0      \\
\hline
STAGG\_SP \cite{DBLP:conf/acl/YihRMCS16}  &  \textbf{71.7} &  -      \\
HR-BiLSTM \cite{DBLP:conf/acl/YuYHSXZ17}                  & 62.3 & 31.2         \\
KBQA-GST \cite{DBLP:conf/ijcai/LanW019}          &  67.9 &  36.5      \\
\hline
Our Method-joint\_prob             &     62.1  &   38.0        \\
Our Method-joint\_prob\_short             &     58.4  &           \\
Our Method-joint\_prob\_random             &     58.8  &           \\
Our Method-joint\_prob\_multiple\_paths             &  63.9     &     -       \\
%Our Method-marginal\_prob\_with\_true\_label             &    \textbf{68.5}    &       34.8     \\
Our Method-marginal\_prob*             &   67.8    &      \textbf{38.4}    \\
%Our Method-obj3+new\_decode  &     &          \\
\hline
\end{tabular}
}
\caption{\fontsize{10}{12}\selectfont We report F1 on WQSP and CWQ. $*$ means this method only requires the final answer as the annotation, and other methods need annotated relation paths or some other annotations.}\label{tab:wqsp_cwq}
\end{table}

\begin{table}[h]\centering
\resizebox{1.01\columnwidth}{!}{
\begin{tabular}{|l|c|c|c|c|}
\hline
                               & \multicolumn{2}{c|}{WQSP}     & \multicolumn{2}{c|}{CWQ}     \\ \hline
                               & 1 path & \textgreater{}1 path & 1 path & \textgreater 1 path \\ \hline
Our Method-joint\_prob         & 60.8   & 63.3                 &    &                \\ 
Our Method-joint\_prob\_short  & 60.0    & 57.0                      &        &                     \\ 
Our Method-joint\_prob\_random &  59.7      &  58.1                    &        &                     \\ 
Our Method-marginal\_prob      & 66.0   & 69.3                 &   &                 \\ \hline
\end{tabular}
}
\caption{\fontsize{10}{12}\selectfont We report F1 on WQSP and CWQ.}\label{tab:wqsp_cwq_path_break}
\end{table}


\begin{table*}[t]\centering
\resizebox{2.1\columnwidth}{!}{%resize the table
\begin{tabular}{l|l|l}
\hline
\multicolumn{3}{c}{Question: what state does romney live in?  \ \ \        Answer: Massachusetts  \ \ \       Topic entity: romney}                                                                                                                                            \\ \hline
.89:children & .29:education\_institution,state\_province\_region & .83:\textbf{places\_lived,location} \\ \hline
.06:\textbf{government\_positions,jurisdiction\_of\_office} & .25:\textbf{places\_lived,location} & .12:\textbf{government\_positions,jurisdiction\_of\_office} \\ \hline
.04:\textbf{government\_positions,office\_position\_or\_title} & .25:\textbf{government\_positions,district\_represented} & .04:\textbf{government\_positions,district\_represented} \\ \hline
.00:\textbf{government\_positions,district\_represented} & .01:\textbf{government\_positions,jurisdiction\_of\_office} & .01:place\_of\_birth,state \\ \hline
.0:place\_of\_birth & .01:place\_of\_birth,state & .00:education,degree \\ \hline
.00:jurisdiction\_of\_office & .01:sibling,place\_of\_birth & .00:election\_campaigns \\ \hline 
\multicolumn{3}{c}{Question:where did madonna grew up?\ \ \       Answer: Bay City\ \ \    Topic entity: madonna}                                                                                                                                            \\ 
\hline
.99:\textbf{place\_of\_birth} & .50:nominated\_for & .47:nominated\_for,featured\_film\_locations \\ \hline
.00:nominated\_for & .16:nominated\_for,featured\_film\_locations & .40:\textbf{place\_of\_birth} \\ \hline
.00:\textbf{place\_lived.location} & .11:compositions & .11:\textbf{place\_lived.location,place} \\ \hline
.00:place\_lived.location,containedby & .09:\textbf{place\_lived.location} & .00:nominated\_for \\ \hline
.00:compositions & .08:\textbf{place\_of\_birth} & .00:\textbf{place\_lived.location} \\ \hline
.00:religion & .01:award\_nominations,nominated\_for & .00:\textbf{place\_lived.location,region} \\ \hline


\end{tabular}
}\caption{\fontsize{10}{12}\selectfont Two running examples from \textsc{WebQuestionSP} dataset. We show the probability $P(\mathbf{r}|q)$ before the inferred relation path. Relation paths that lead to the correct answers are highlighted in bold. The three columns are corresponding to the results by using joint objective with single path, joint objective with multiple paths, and marginal objective with multiple paths. Due to space limit, we only show the partial name of a relation in the example and the probability less than .01 is shown as .00.}\label{tab:case}
\end{table*}

\subsubsection{ComplexWebQuestion-1.1}

This dataset is designed to study complex questions by adding more constraints to questions in \textsc{WebQuestionSP}. It contains more difficult questions than the first two datasets.  We report the experimental results in Table \ref{tab:wqsp_cwq}. Note that this dataset does not come with multiple relation path labels, so the corresponding experiment is not available. Our model outperforms all other models in terms of hits@1, and slightly worse than KBQA-GST in terms of F1 score, but again, KBQA-GST requires many additional information to train. Different from the observation in \textsc{WebQuestionSP} dataset, we see that there is a performance degradation when the model is not pre-trained with ground truth relations. It is because that the model can easily make errors in early stage and gets stuck with these errors. In contrast, our model on WQSP does not suffer from this problem because the relation path is much shorter, and thus it is not hard to generate correct training samples at the beginning of the training. To compare it with existing methods, our model still performs better than GRAFT-Net, which is the state-of-the-art results without using any additional labels.


\begin{table*}[t]\centering
\resizebox{2.1\columnwidth}{!}{%resize the table
\begin{tabular}{l|l|l}
\hline
\multicolumn{3}{c}{Question: what state does romney live in?  \ \ \        Answer: Massachusetts  \ \ \       Topic entity: romney}                                                                                                                                            \\ \hline
\textsc{Single\ Ground\ truth} & \textsc{Multiple\ product} & \textsc{Multiple\ summation (our)}\\ \hline
.89:children & .29:education\_institution/\ state\_province\_region & .83:\textbf{places\_lived/\ location} \\ \hline
.06:\textbf{government\_positions/\ jurisdiction\_of\_office} & .25:\textbf{places\_lived/\ location} & .12:\textbf{government\_positions/\ jurisdiction\_of\_office} \\ \hline
.04:\textbf{government\_positions/\ office\_position\_or\_title} & .25:\textbf{government\_positions/\ district\_represented} & .04:\textbf{government\_positions/\ district\_represented} \\ \hline
.00:\textbf{government\_positions/\ district\_represented} & .01:\textbf{government\_positions/\ jurisdiction\_of\_office} & .01:place\_of\_birth/\ state \\ \hline
.00:place\_of\_birth & .01:place\_of\_birth/\ state & .00:education/\ degree \\ \hline
.00:jurisdiction\_of\_office & .01:sibling/\ place\_of\_birth & .00:election\_campaigns \\ \hline 
\multicolumn{3}{c}{Question:where did madonna grew up?\ \ \       Answer: Bay City\ \ \    Topic entity: madonna}                                                                                                                                            \\ 
\hline
\textsc{Single\ Ground\ truth} & \textsc{Multiple\ product} & \textsc{Multiple\ summation (our)}\\ \hline
.99:\textbf{place\_of\_birth} & .50:nominated\_for & .47:nominated\_for/\ featured\_film\_locations \\ \hline
.00:nominated\_for & .16:nominated\_for/\ featured\_film\_locations & .40:\textbf{place\_of\_birth} \\ \hline
.00:\textbf{place\_lived.location} & .11:compositions & .11:\textbf{place\_lived.location/\ place} \\ \hline
.00:place\_lived.location/\ containedby & .09:\textbf{place\_lived.location} & .00:nominated\_for \\ \hline
.00:compositions & .08:\textbf{place\_of\_birth} & .00:\textbf{place\_lived.location} \\ \hline
.00:religion & .01:award\_nominations/\ nominated\_for & .00:\textbf{place\_lived.location/\ region} \\ \hline


\end{tabular}
}\caption{\fontsize{10}{12}\selectfont Two running examples from \textsc{WebQuestionSP} dataset. We show the probability $P(r_0,...,r_T|q)$ before the inferred relation path. Paths that lead to the correct answers are highlighted in bold. We use $/$ to split two relations. The three columns are corresponding to the results by using different training settings as it is in Table \ref{tab:obj_fcn}: single ground truth, multiple product, and multiple summation (our). Due to space limit, we only show the partial name of a relation in the example and the probability less than .01 is shown as .00. We do not show $P(e_0,...,e_{T-1}|q)$ because they are not determined by our model. }\label{tab:case}
\end{table*}
